SMASH: Co-designing Software Compression and Hardware-Accelerated Indexing for Efficient Sparse Matrix Operations

Important workloads, such as machine learning and graph analytics applications, heavily involve sparse linear algebra operations. These operations use sparse matrix compression as an effective means to avoid storing zeros and performing unnecessary computation on zero elements. However, compression techniques like Compressed Sparse Row (CSR) that are widely used today introduce significant instruction overhead and expensive pointer-chasing operations to discover the positions of the non-zero elements. In this paper, we identify the discovery of the positions (i.e., indexing) of non-zero elements as a key bottleneck in sparse matrix-based workloads, which greatly reduces the benefits of compression. We propose SMASH, a hardware-software cooperative mechanism that enables highly-efficient indexing and storage of sparse matrices. The key idea of SMASH is to explicitly enable the hardware to recognize and exploit sparsity in data. To this end, we devise a novel software encoding based on a hierarchy of bitmaps. This encoding can be used to efficiently compress any sparse matrix, regardless of the extent and structure of sparsity. At the same time, the bitmap encoding can be directly interpreted by the hardware. We design a lightweight hardware unit, the Bitmap Management Unit (BMU), that buffers and scans the bitmap hierarchy to perform highly-efficient indexing of sparse matrices. SMASH exposes an expressive and rich ISA to communicate with the BMU, which enables its use in accelerating any sparse matrix computation. We demonstrate the benefits of SMASH on four use cases that include sparse matrix kernels and graph analytics applications.

==> Makefile <==
PDF = smash.pdf

all: ${PDF}

smash.pdf: main.tex acmart.cls ACM-Reference-Format.bst
	pdflatex --shell-escape main.tex 
	bibtex main.aux
	pdflatex --shell-escape main.tex
	pdflatex --shell-escape main.tex
clean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.gz *.zip *.rpi \
  $(PDF) *-converted-to.pdf


==> abstract-nv.tex <==


Important workloads, such as machine learning and graph analytics applications, heavily involve sparse linear algebra operations.
These operations use sparse matrix compression as an effective way to avoid storing zeros and performing unnecessary computations. However, prevalent compression techniques such as Compressed Sparse Row (CSR) either suffer from significant computation overhead as a result of the compression scheme, or are highly tailored certain types of sparse matrices and are not general in applicability.
%introduce significant instruction overhead to discover the positions of the non-zero elements. 
In this paper, we identify the discovery of the positions (i.e., indexing) of non-zero elements as a key bottleneck in sparse matrix compression schemes that are used today, which greatly reduces the benefits of compression.  

We propose SMASH, a hardware/software cooperative mechanism that addresses this bottleneck via the combination of sparse matrix software compression and efficient hardware-accelerated indexing. On the software side, SMASH uses a novel hierarchy of bitmaps to identify regions of the sparse matrix that contain zero or non-zero elements. %This hierarchy compresses information about the positions of non-zero elements of the sparse matrix with affordable storage overhead. 
On the hardware side, a lightweight hardware accelerator, called Bitmap Management Unit (BMU), buffers and scans the bitmap hierarchy to perform efficient indexing.  SMASH exposes an expressive and rich ISA to communicate with the BMU, which enables its use in many sparse matrix kernels.

%We introduce two software data structures to efficiently compress sparse matrices, and we extend hardware to accelerate the indexing of the non-zero elements of the matrix. SMASH consists of a bitmap-based compression format to keep track of the non-zero cache lines of the matrix, and a data structure that efficiently compresses its values. At the hardware level, it provides an expressive ISA  and a bitmap buffering mechanism to enable low-cost indexing of the non-zero elements. SMASH can also be reconfigured to encode information at multiple granularities.



==> discussion.tex <==
\section{Discussion}\label{Discussionbl}
%In this work, we evaluate SMASH only for SpMM and SpMV kernels, which are the most performance-critical kernels for a large number of applications. However, SMASH is a generally applicable mechanism that can be used to accelerate various sparse matrix kernels. Performing Sparse Matrix operations requires 1) the non-zero values of the elements in the matrix, and 2) the indices -row and column- of those elements.






==> motivation.tex <==
\section{Motivation}
\label{Motivationlbl}

%Many important applications ranging from Sparse Linear Algebra operations and Graph Processing~\cite{van2008graph, bulucc2012parallel, penn2006efficient} to Convolutional Neural Networks (CNNs)~\cite{liu2015sparse} and Machine Learning (ML)~\cite{zhao2018bridging} commonly use Sparse Matrix-Vector Multiplication (SpMV) and Sparse Matrix-Matrix Multiplication (SpMM) operations. 
\begin{comment}
 Generally, SpMV is  repetitive within iterative solvers and graph computations, making it a performance-critical component whose overhead can dominate overall application running time.
 More specifically, SpMV is predominant across different applications, like PageRank\cite{}, Betweeness-Centrality\cite{} and Minimum spanning tree\cite{}.
 
 On the other hand, SpMM is a crucial building block of multiple algorithms spanning from graph analytics to linear algebra solvers. Batch evaluation of pruned CNNs \cite{}, Breadth-First Search \cite{}, Markov clustering \cite{} and Shur's complement method \cite{} are some examples where SpMM dominates the end-to-end execution time. Other methods like finite element simulations also rely on sparse matrix-matrix multiplication.

\end{comment}
%A large portion of the data structures involved in these application Operations involve zero elements. Thus, a common approach to reduce both computational and storage overheads is to use compression techniques. However, as discussed in Section \ref{Introductionlbl}, sparse matrix compression faces several challenges.

Sparse Matrix Operations are widely used to a variety of applications ranging from Sparse Linear Algebra and Graph Processing~\cite{van2008graph, bulucc2012parallel, penn2006efficient} to Convolutional Neural Networks (CNNs)~\cite{liu2015sparse} and Machine Learning (ML)~\cite{zhao2018bridging}. As already mentioned, the matrices involved in these applications include a lot of zero elements and thus, a common approach to avoid needless computations and reduce storage overheads is to use compressed format representations for sparse matrices. However, Sparse Matrix Operations face several challenges. 


%A large body of prior works, like CSR \cite{barrett1994templates, saad2003iterative}, BCSR \cite{pinar1999improving, im2001optimizing}, CSR5 \cite{Liu2015WanEff}, and \cite{Nurvitadhi2015asparse}, focuses on reducing the storage space of the compressed data and avoiding redundant computation on zero elements of the matrix  (Challenge 1) while being applicable to different formats of these data structures (Challenge 3). However, these schemes do not address Challenge 2 and require storing the indices of non-zero elements in memory (see Section \ref{csr_description}). This means that these mechanisms access memory to retrieve the row and column addresses of the non-zero elements. Even BCSR \cite{pinar1999improving, im2001optimizing} requires additional accesses to find out the positions of the blocks. This increases the memory traffic and lowers the potential gains from compressing and avoiding computation. Figure~\ref{fig:Optimal_indexing} shows the number of instructions and the execution time of an optimal indexing scenario in which accessing the indices of non-zero elements does not incur additional computation. These numbers are normalized to the number of instructions and the execution time of CSR, respectively. This shows that addressing Challenge 2 has the potential of increasing performance by up to $2.81\times$ for SpMM and $2.13\times$ for SpMV. The reduction in the number of instructions in the optimal indexing case justifies this performance gain. 




Prior works propose compressed storage formats like  CSR \cite{barrett1994templates, saad2003iterative}, BCSR \cite{blockoptim1999, im2001optimizing}, CSR5 \cite{Liu2015WanEff}, and only focus on addressing Challenge 1, by reducing the storage area and avoiding redundant computations on zero elements of the matrix, while some of them being applicable to different Sparse Matrix Operations (Challenge 3). However, none of those works does address Challenge 2 resulting in additional memory accesses needed to find the indices, i.e. the row and column addresses of non-zero elements. Consequently, this increases the memory traffic and lowers the potential gains from compressing and avoiding computation. Figure~\ref{fig:Optimal_indexing} shows the number of instructions and the execution time of an optimal indexing scenario in which accessing the indices of non-zero elements does not incur any additional computation. As shown in this figure, addressing Challenge 2 significantly increases the number of instructions, and results in high performance improvement, i.e. a performance speedup up to $2.81\times$ for SpMM, $2.13\times$ for SpMV kernel and $2.21\times$ for Sparse Matrix Addition. 

%\begin{figure}[t]
%    \begin{subfigure}[b]{.21\textwidth}
    %\captionsetup{justification=centering}
%                \centering
%                \includegraphics[scale = 0.8]{figures/csr_optimal_indexing.pdf}
%                 \vspace{-3mm}
%                 \caption{\hspace*{-4em}}
%    \end{subfigure}%
%    \begin{subfigure}[b]{.30\textwidth}
%        %\captionsetup{justification=centering}
%            \centering
%            \includegraphics[scale = 0.8]{figures/csr_optimal_indexing_inst.pdf}
%           \vspace{-3mm}
%            \caption{\hspace*{-4em}}
%    \end{subfigure}
%    \vspace{-5mm}
%     \caption{Performance and number of instructions of an optimal indexing scheme for SpMV, SpMM and Sparse Matrix Addition over  baseline CSR. Results average across 25 sparse matrices.}
%         \label{fig:Optimal_indexing}
%\vspace{-6mm}
%\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[scale = 1.0]{figures/optimal_indexing.pdf}
    \vspace{-5mm}
     \caption{Speedup and number of instructions of an optimal indexing scheme for Sparse Matrix Addition, SpMV and SpMM over  baseline CSR. Results average across 25 sparse matrices.}
    \label{fig:Optimal_indexing}
\end{figure}

%The other class of prior works addresses Challenges 1 and 2, while assuming a specific matrix structure. For example, some works \cite{saad2003iterative} assume diagonal format for the matrices, while others build on the assumption of matrices having few unique non-zero elements \cite{unique}. Their solutions are not applicable to matrices with different structures (Challenge 3). Important application classes like Neural Network Inference and Graph Processing use general matrices which are not necessarily diagonal, and do not have repeated unique numbers. This makes this class of compression techniques not suitable for these applications. 

%In this work, we aim to tackle all the three challenges by combining software compression and hardware-accelerated indexing, in a mechanism that we call SMASH. 

Finally, even though there are prior works that address both Challenge 1 and 2, lack generality (Challenge 3) and assume a specific matrix structure. Saad et al. ~\cite{saad2003iterative} assume a diagonal matrix, while Kourtis et al. ~\cite{unique} assume matrices of few unique non-zero elements. However, many classes of applications like Convolutional Neural Networks and Graph Processing algorithms involve matrices which are not necessarily diagonal or do not have a repeated value pattern. This makes these prior works not suitable for these applications. On the other hand, in our work, we aim to tackle all three Challenges associated with Sparse Matrix Operations and thus, we combine software compression with hardware-accelerated indexing, in a mechanism called SMASH.

%\vspace{-2.5mm}



==> out <==
pdflatex --shell-escape main.tex 
This is pdfTeX, Version 3.14159265-2.6-1.40.19 (TeX Live 2019/dev/Debian) (preloaded format=pdflatex)
 \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2018-12-01>
(./acmart.cls
Document Class: acmart 2019/04/22 v1.60 Typesetting articles for the Associatio
n for Computing Machinery
(/usr/share/texlive/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/xkvutils.tex
(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/keyval.tex))))
(/usr/share/texlive/texmf-dist/tex/generic/xstring/xstring.sty
(/usr/share/texlive/texmf-dist/tex/generic/xstring/xstring.tex))
(/usr/share/texlive/texmf-dist/tex/latex/amscls/amsart.cls
Document Class: amsart 2017/10/31 v2.20.4
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/share/texlive/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/refcount.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ltxcmds.sty)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/infwarerr.sty))
(/usr/share/texlive/texmf-dist/tex/latex/totpages/totpages.sty
(/usr/share/texlive/texmf-dist/tex/latex/ms/everyshi.sty))
(/usr/share/texlive/texmf-dist/tex/latex/environ/environ.sty
(/usr/share/texlive/texmf-dist/tex/latex/trimspaces/trimspaces.sty))
(/usr/share/texlive/texmf-dist/tex/latex/textcase/textcase.sty)
(/usr/share/texlive/texmf-dist/tex/latex/natbib/natbib.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/share/texlive/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/share/texlive/texmf-dist/tex/latex/url/url.sty))
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texlive/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/share/texlive/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/geometry/geometry.sty)
(/usr/share/texlive/texmf-dist/tex/latex/ncctools/manyfoot.sty
(/usr/share/texlive/texmf-dist/tex/latex/ncctools/nccfoots.sty))
(/usr/share/texlive/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/share/texlive/texmf-dist/tex/generic/pdftex/glyphtounicode.tex)
(/usr/share/texlive/texmf-dist/tex/latex/cmap/cmap.sty)
(/usr/share/texlive/texmf-dist/tex/latex/base/fontenc.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/t1enc.def)<<t1.cmap>>)
(/usr/share/texlive/texmf-dist/tex/latex/libertine/libertine.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/textcomp.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/ts1enc.def
(/usr/share/texlive/texmf-dist/tex/latex/base/ts1enc.dfu)))
(/usr/share/texlive/texmf-dist/tex/latex/mweights/mweights.sty)
(/usr/share/texlive/texmf-dist/tex/latex/base/fontenc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/fontaxes/fontaxes.sty)
(/usr/share/texlive/texmf-dist/tex/latex/libertine/LinLibertine_I.tex))
(/usr/share/texlive/texmf-dist/tex/latex/inconsolata/zi4.sty
`inconsolata-zi4' v1.112, 2017/01/04 Text macros for Inconsolata (msharpe))
(/usr/share/texlive/texmf-dist/tex/latex/newtx/newtxmath.sty
`newtxmath' v1.553, 2018/05/15 Math macros based originally on txfonts (msharpe
) (/usr/share/texlive/texmf-dist/tex/latex/oberdiek/centernot.sty)
(/usr/share/texlive/texmf-dist/tex/generic/kastrup/binhex.tex))
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption.sty
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption3.sty))
(/usr/share/texlive/texmf-dist/tex/latex/float/float.sty)
(/usr/share/texlive/texmf-dist/tex/latex/comment/comment.sty
Excluding comment 'comment') Excluding comment 'CCSXML'
(/usr/share/texlive/texmf-dist/tex/latex/fancyhdr/fancyhdr.sty)
Special comment 'acks'
(/usr/share/texlive/texmf-dist/tex/latex/libertine/T1LinuxLibertineT-TLF.fd))
(/usr/share/texlive/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/share/texlive/texmf-dist/tex/latex/tools/calc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/share/texlive/texmf-dist/tex/latex/setspace/setspace.sty)
(/usr/share/texlive/texmf-dist/tex/latex/algorithms/algorithm.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/ifthen.sty))
(/usr/share/texlive/texmf-dist/tex/latex/algorithms/algorithmic.sty)
(/usr/share/texlive/texmf-dist/tex/latex/caption/subcaption.sty)
(/usr/share/texlive/texmf-dist/tex/latex/tools/array.sty)
(/usr/share/texlive/texmf-dist/tex/generic/ulem/ulem.sty)
(/usr/share/texlive/texmf-dist/tex/latex/minted/minted.sty
(/usr/share/texlive/texmf-dist/tex/latex/fvextra/fvextra.sty
(/usr/share/texlive/texmf-dist/tex/latex/fancyvrb/fancyvrb.sty
Style option: `fancyvrb' v3.2a <2019/01/15> (tvz))
(/usr/share/texlive/texmf-dist/tex/latex/upquote/upquote.sty)
(/usr/share/texlive/texmf-dist/tex/latex/lineno/lineno.sty))
(/usr/share/texlive/texmf-dist/tex/latex/tools/shellesc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/ifplatform/ifplatform.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/catchfile.sty) (./main.w18)
) (/usr/share/texlive/texmf-dist/tex/latex/framed/framed.sty)
(/usr/share/texlive/texmf-dist/tex/latex/caption/newfloat.sty))
(/usr/share/texlive/texmf-dist/tex/latex/tools/hhline.sty)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/frontendlayer/tikz.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-common-lists.t
ex)) (/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def
) (/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/pgf.revision.tex)))
(/usr/share/texlive/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeysfiltered.code.t
ex)) (/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.def
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-pdf.de
f)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.code.
tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigonomet
ric.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.random.cod
e.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.comparison
.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integerari
thmetics.code.tex)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconstruct.
code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicstate.c
ode.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransformation
s.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.code.tex
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.code.t
ex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathprocessing
.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.code.tex
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.code.tex

(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.code.
tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransparency.c
ode.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorerdf.code.tex))
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.code.tex
) (/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.tex
)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-0-65
.sty)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-1-18
.sty)) (/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgffor.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgfkeys.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex))
(/usr/share/texlive/texmf-dist/tex/latex/pgf/math/pgfmath.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgffor.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/tikz.code.tex

(/usr/share/texlive/texmf-dist/tex/generic/pgf/libraries/pgflibraryplothandlers
.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmodulematrix.code.tex
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tik
zlibrarytopaths.code.tex)))
(/usr/share/texlive/texmf-dist/tex/latex/mdframed/mdframed.sty
(/usr/share/texlive/texmf-dist/tex/latex/l3packages/xparse/xparse.sty
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/expl3.sty
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/expl3-code.tex)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3pdfmode.def)))
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/zref-abspage.sty
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/zref-base.sty))
(/usr/share/texlive/texmf-dist/tex/latex/needspace/needspace.sty)
(/usr/share/texlive/texmf-dist/tex/latex/mdframed/md-frame-0.mdf))
(/usr/share/texlive/texmf-dist/tex/latex/makecell/makecell.sty)
(/usr/share/texlive/texmf-dist/tex/latex/dblfloatfix/dblfloatfix.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

)) (/usr/share/texlive/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/share/texlive/texmf-dist/tex/latex/tools/afterpage.sty)
(/usr/share/texlive/texmf-dist/tex/latex/listings/listings.sty
(/usr/share/texlive/texmf-dist/tex/latex/listings/lstmisc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/listings/listings.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/listings/lstlang1.sty)
(/usr/share/texlive/texmf-dist/tex/latex/preprint/balance.sty)
Excluding comment 'screenonly' Include comment 'printonly'
Include comment 'anonsuppress'/usr/bin/pygmentize
 (./main.aux)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/omlnxlmi.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/untxexa.fd)
(/usr/share/texlive/texmf-dist/tex/latex/base/ts1cmr.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/lmsntxsy.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/lmxntxexx.fd)
(/usr/share/texlive/texmf-dist/tex/latex/libertine/OT1LinuxLibertineT-TLF.fd)<<
ot1.cmap>><<oml.cmap>>
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/untxmia.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/untxsym.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/untxsyc.fd)
ABD: EveryShipout initializing macros
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))
(./main.out) (./main.out)
(/usr/share/texlive/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texlive/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(/usr/share/texlive/texmf-dist/tex/latex/libertine/T1LinuxBiolinumT-TLF.fd)
(/usr/share/texlive/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/microtype/mt-msb.cfg) (./abstract.tex
Excluding 'comment' comment.)

Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `\\' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `\\' on input line 158.

(./introduction.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 2.


Underfull \vbox (badness 5036) has occurred while \output is active [1.1{/var/l
ib/texmf/fonts/map/pdftex/updmap/pdftex.map}]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 47.


Underfull \vbox (badness 10000) has occurred while \output is active)
(./background.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 15.

(/usr/share/texlive/texmf-dist/tex/latex/inconsolata/t1zi4.fd)

pdfTeX warning: pdflatex (file ./csr.pdf): PDF inclusion: found PDF version <1.
7>, but at most version <1.5> allowed

Class acmart Warning: A possible image without description on input line 30.


LaTeX Warning: `!h' float specifier changed to `!ht'.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 35.

[2.2]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 42.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 42.

(./main.out.pyg) (./main.out.pyg) (./main.out.pyg)

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 48.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 74.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 74.

(./main.out.pyg)

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 84.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 86.



pdfTeX warning: pdflatex (file ./index_matching.pdf): PDF inclusion: found PDF 
version <1.7>, but at most version <1.5> allowed

Overfull \hbox (26.59892pt too wide) in paragraph at lines 93--96
 []|  [] 

Class acmart Warning: A possible image without description on input line 99.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 103.


Class acmart Warning: A possible image without description on input line 116.

[3.3 <./csr.pdf> <./index_matching.pdf

pdfTeX warning: pdflatex (file ./index_matching.pdf): PDF inclusion: multiple p
dfs with page group included in a single page
>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 121.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 123.

) (./overview.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 7.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 10.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 19.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 21.



pdfTeX warning: pdflatex (file ./overview_bitmap.pdf): PDF inclusion: found PDF
 version <1.7>, but at most version <1.5> allowed

Overfull \hbox (31.99515pt too wide) in paragraph at lines 29--32
 []|  [] 

Class acmart Warning: A possible image without description on input line 35.


LaTeX Warning: `!h' float specifier changed to `!ht'.


Underfull \vbox (badness 4001) has occurred while \output is active [4.4 <./opt
imal_indexing.pdf>]) (./mechanism.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 9.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 12.



pdfTeX warning: pdflatex (file ./bitmap_final.pdf): PDF inclusion: found PDF ve
rsion <1.7>, but at most version <1.5> allowed

Class acmart Warning: A possible image without description on input line 37.

[5.5 <./overview_bitmap.pdf> <./bitmap_final.pdf

pdfTeX warning: pdflatex (file ./bitmap_final.pdf): PDF inclusion: multiple pdf
s with page group included in a single page
>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 113.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `\newline' on input line 114.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 120.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 126.



pdfTeX warning: pdflatex (file ./bmu_overview.pdf): PDF inclusion: found PDF ve
rsion <1.7>, but at most version <1.5> allowed

Overfull \hbox (17.5091pt too wide) in paragraph at lines 134--137
 []|  [] 

Class acmart Warning: A possible image without description on input line 140.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 141.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 152.

[6.6 <./bmu_overview.pdf>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 187.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 253.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 255.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 287.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 290.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 292.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 294.



pdfTeX warning: pdflatex (file ./flow_spmv.pdf): PDF inclusion: found PDF versi
on <1.7>, but at most version <1.5> allowed

Class acmart Warning: A possible image without description on input line 313.


LaTeX Warning: `!h' float specifier changed to `!ht'.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 318.


Overfull \hbox (3.25229pt too wide) in paragraph at lines 334--335
[][][][][][][][][][][][][][][][][][][][][][]  

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 337.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 339.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 339.


LaTeX Warning: `!h' float specifier changed to `!ht'.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 357.

[7.7]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 433.


Underfull \vbox (badness 3514) has occurred while \output is active

pdfTeX warning: pdflatex (file ./flow_spmm.pdf): PDF inclusion: found PDF versi
on <1.7>, but at most version <1.5> allowed

Class acmart Warning: A possible image without description on input line 453.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 458.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 476.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 478.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 478.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 480.

) (./evaluation.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 4.


LaTeX Warning: `h' float specifier changed to `ht'.


LaTeX Warning: `h' float specifier changed to `ht'.


LaTeX Warning: `h' float specifier changed to `ht'.

[8.8 <./flow_spmv.pdf> <./flow_spmm.pdf

pdfTeX warning: pdflatex (file ./flow_spmm.pdf): PDF inclusion: multiple pdfs w
ith page group included in a single page
>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 141.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 162.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 165.


Class acmart Warning: A possible image without description on input line 191.


LaTeX Warning: `h' float specifier changed to `ht'.

[9.9]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 224.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 227.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 234.


Class acmart Warning: A possible image without description on input line 244.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 245.


Class acmart Warning: A possible image without description on input line 255.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 275.


Class acmart Warning: A possible image without description on input line 285.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 287.


Class acmart Warning: A possible image without description on input line 297.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 341.

[10.10 <./software.pdf> <./speedup_SpMV.pdf> <./instructions_SpMV.pdf> <./speed
up_SpMM.pdf> <./instructions_SpMM.pdf>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 371.


Class acmart Warning: A possible image without description on input line 382.


Class acmart Warning: A possible image without description on input line 391.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 406.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 423.


Class acmart Warning: A possible image without description on input line 432.


Class acmart Warning: A possible image without description on input line 441.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 518.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 521.


Class acmart Warning: A possible image without description on input line 537.

[11.11 <./granularity_spmv.pdf> <./granularity_spmm.pdf> <./locality_spmv.pdf> 
<./locality_spmm.pdf>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 555.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 557.


Class acmart Warning: A possible image without description on input line 573.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 611.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 614.


Class acmart Warning: A possible image without description on input line 632.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 653.

[12.12 <./graph.pdf> <./storage.pdf> <./conversion.pdf>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 656.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 666.

Excluding 'comment' comment.) (./related_work.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.

) (./conclusion.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.

[13.13]) (./acknowledgements.tex) (./main.bbl [14.14])

Class acmart Warning: Some images may lack descriptions.


Package balance Warning: You have called \balance in second column
(balance)                Columns might not be balanced.

[15.15] (./main.aux) )
(see the transcript file for additional information)pdfTeX warning (dest): name
{Hfootnote.1} has been referenced but does not exist, replaced by a fixed one

pdfTeX warning (dest): name{lstnumber.-2.17} has been referenced but does not e
xist, replaced by a fixed one

{/usr/share/texlive/texmf-dist/fonts/enc/dvips/newtx/libertinealt.enc}{/usr/sha
re/texlive/texmf-dist/fonts/enc/dvips/libertine/lbtn_25tcsq.enc}{/usr/share/tex
live/texmf-dist/fonts/enc/dvips/inconsolata/i4-t1-4.enc}{/usr/share/texlive/tex
mf-dist/fonts/enc/dvips/base/8r.enc}{/usr/share/texlive/texmf-dist/fonts/enc/dv
ips/libertine/lbtn_7grukw.enc}{/usr/share/texlive/texmf-dist/fonts/enc/dvips/li
bertine/lbtn_nh77jq.enc}{/usr/share/texlive/texmf-dist/fonts/enc/dvips/libertin
e/lbtn_oexx6f.enc}{/usr/share/texlive/texmf-dist/fonts/enc/dvips/libertine/lbtn
_76gpa5.enc}</usr/share/texlive/texmf-dist/fonts/type1/public/inconsolata/Incon
solata-zi4b.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/inconsolata/I
nconsolata-zi4r.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine
/LinBiolinumTB.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine/
LinBiolinumTI.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine/L
inLibertineT.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine/Li
nLibertineTB.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine/Li
nLibertineTI.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/newtx/fxlri-
7letters.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/txfonts/rtxmi.pf
b></usr/share/texlive/texmf-dist/fonts/type1/public/txfonts/rtxr.pfb></usr/shar
e/texlive/texmf-dist/fonts/type1/public/newtx/txexs.pfb></usr/share/texlive/tex
mf-dist/fonts/type1/public/newtx/txsys.pfb></usr/share/texlive/texmf-dist/fonts
/type1/public/newtx/zxlri.pfb>
Output written on main.pdf (15 pages, 1267602 bytes).
Transcript written on main.log.
bibtex main.aux
This is BibTeX, Version 0.99d (TeX Live 2019/dev/Debian)
The top-level auxiliary file: main.aux
The style file: IEEEtranS.bst.bst
Database file #1: refs.bib
-- IEEEtranS.bst version 1.13 (2008/09/30) by Michael Shell.
-- http://www.michaelshell.org/tex/ieeetran/bibtex/
-- See the "IEEEtran_bst_HOWTO.pdf" manual for usage information.
** Sorting version - not for normal IEEE work.
Warning--to sort, need author or key in intel-mkl
Warning--to sort, need author or key in intelxeon
Warning--to sort, need author or key in smash
Warning--empty booktitle in pei2015
Warning--empty booktitle in googleworkloads2018
Warning--empty journal in dongarra1996sparse
Warning--empty booktitle in impica2016
Warning--missing publisher in saad2003iterative

Done.
(There were 8 warnings)
pdflatex --shell-escape main.tex
This is pdfTeX, Version 3.14159265-2.6-1.40.19 (TeX Live 2019/dev/Debian) (preloaded format=pdflatex)
 \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2018-12-01>
(./acmart.cls
Document Class: acmart 2019/04/22 v1.60 Typesetting articles for the Associatio
n for Computing Machinery
(/usr/share/texlive/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/xkvutils.tex
(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/keyval.tex))))
(/usr/share/texlive/texmf-dist/tex/generic/xstring/xstring.sty
(/usr/share/texlive/texmf-dist/tex/generic/xstring/xstring.tex))
(/usr/share/texlive/texmf-dist/tex/latex/amscls/amsart.cls
Document Class: amsart 2017/10/31 v2.20.4
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/share/texlive/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/refcount.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ltxcmds.sty)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/infwarerr.sty))
(/usr/share/texlive/texmf-dist/tex/latex/totpages/totpages.sty
(/usr/share/texlive/texmf-dist/tex/latex/ms/everyshi.sty))
(/usr/share/texlive/texmf-dist/tex/latex/environ/environ.sty
(/usr/share/texlive/texmf-dist/tex/latex/trimspaces/trimspaces.sty))
(/usr/share/texlive/texmf-dist/tex/latex/textcase/textcase.sty)
(/usr/share/texlive/texmf-dist/tex/latex/natbib/natbib.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/share/texlive/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/share/texlive/texmf-dist/tex/latex/url/url.sty))
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texlive/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/share/texlive/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/geometry/geometry.sty)
(/usr/share/texlive/texmf-dist/tex/latex/ncctools/manyfoot.sty
(/usr/share/texlive/texmf-dist/tex/latex/ncctools/nccfoots.sty))
(/usr/share/texlive/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/share/texlive/texmf-dist/tex/generic/pdftex/glyphtounicode.tex)
(/usr/share/texlive/texmf-dist/tex/latex/cmap/cmap.sty)
(/usr/share/texlive/texmf-dist/tex/latex/base/fontenc.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/t1enc.def)<<t1.cmap>>)
(/usr/share/texlive/texmf-dist/tex/latex/libertine/libertine.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/textcomp.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/ts1enc.def
(/usr/share/texlive/texmf-dist/tex/latex/base/ts1enc.dfu)))
(/usr/share/texlive/texmf-dist/tex/latex/mweights/mweights.sty)
(/usr/share/texlive/texmf-dist/tex/latex/base/fontenc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/fontaxes/fontaxes.sty)
(/usr/share/texlive/texmf-dist/tex/latex/libertine/LinLibertine_I.tex))
(/usr/share/texlive/texmf-dist/tex/latex/inconsolata/zi4.sty
`inconsolata-zi4' v1.112, 2017/01/04 Text macros for Inconsolata (msharpe))
(/usr/share/texlive/texmf-dist/tex/latex/newtx/newtxmath.sty
`newtxmath' v1.553, 2018/05/15 Math macros based originally on txfonts (msharpe
) (/usr/share/texlive/texmf-dist/tex/latex/oberdiek/centernot.sty)
(/usr/share/texlive/texmf-dist/tex/generic/kastrup/binhex.tex))
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption.sty
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption3.sty))
(/usr/share/texlive/texmf-dist/tex/latex/float/float.sty)
(/usr/share/texlive/texmf-dist/tex/latex/comment/comment.sty
Excluding comment 'comment') Excluding comment 'CCSXML'
(/usr/share/texlive/texmf-dist/tex/latex/fancyhdr/fancyhdr.sty)
Special comment 'acks'
(/usr/share/texlive/texmf-dist/tex/latex/libertine/T1LinuxLibertineT-TLF.fd))
(/usr/share/texlive/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/share/texlive/texmf-dist/tex/latex/tools/calc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/share/texlive/texmf-dist/tex/latex/setspace/setspace.sty)
(/usr/share/texlive/texmf-dist/tex/latex/algorithms/algorithm.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/ifthen.sty))
(/usr/share/texlive/texmf-dist/tex/latex/algorithms/algorithmic.sty)
(/usr/share/texlive/texmf-dist/tex/latex/caption/subcaption.sty)
(/usr/share/texlive/texmf-dist/tex/latex/tools/array.sty)
(/usr/share/texlive/texmf-dist/tex/generic/ulem/ulem.sty)
(/usr/share/texlive/texmf-dist/tex/latex/minted/minted.sty
(/usr/share/texlive/texmf-dist/tex/latex/fvextra/fvextra.sty
(/usr/share/texlive/texmf-dist/tex/latex/fancyvrb/fancyvrb.sty
Style option: `fancyvrb' v3.2a <2019/01/15> (tvz))
(/usr/share/texlive/texmf-dist/tex/latex/upquote/upquote.sty)
(/usr/share/texlive/texmf-dist/tex/latex/lineno/lineno.sty))
(/usr/share/texlive/texmf-dist/tex/latex/tools/shellesc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/ifplatform/ifplatform.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/catchfile.sty) (./main.w18)
) (/usr/share/texlive/texmf-dist/tex/latex/framed/framed.sty)
(/usr/share/texlive/texmf-dist/tex/latex/caption/newfloat.sty))
(/usr/share/texlive/texmf-dist/tex/latex/tools/hhline.sty)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/frontendlayer/tikz.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-common-lists.t
ex)) (/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def
) (/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/pgf.revision.tex)))
(/usr/share/texlive/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeysfiltered.code.t
ex)) (/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.def
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-pdf.de
f)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.code.
tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigonomet
ric.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.random.cod
e.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.comparison
.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integerari
thmetics.code.tex)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconstruct.
code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicstate.c
ode.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransformation
s.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.code.tex
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.code.t
ex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathprocessing
.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.code.tex
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.code.tex

(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.code.
tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransparency.c
ode.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorerdf.code.tex))
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.code.tex
) (/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.tex
)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-0-65
.sty)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-1-18
.sty)) (/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgffor.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgfkeys.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex))
(/usr/share/texlive/texmf-dist/tex/latex/pgf/math/pgfmath.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgffor.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/tikz.code.tex

(/usr/share/texlive/texmf-dist/tex/generic/pgf/libraries/pgflibraryplothandlers
.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmodulematrix.code.tex
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tik
zlibrarytopaths.code.tex)))
(/usr/share/texlive/texmf-dist/tex/latex/mdframed/mdframed.sty
(/usr/share/texlive/texmf-dist/tex/latex/l3packages/xparse/xparse.sty
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/expl3.sty
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/expl3-code.tex)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3pdfmode.def)))
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/zref-abspage.sty
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/zref-base.sty))
(/usr/share/texlive/texmf-dist/tex/latex/needspace/needspace.sty)
(/usr/share/texlive/texmf-dist/tex/latex/mdframed/md-frame-0.mdf))
(/usr/share/texlive/texmf-dist/tex/latex/makecell/makecell.sty)
(/usr/share/texlive/texmf-dist/tex/latex/dblfloatfix/dblfloatfix.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

)) (/usr/share/texlive/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/share/texlive/texmf-dist/tex/latex/tools/afterpage.sty)
(/usr/share/texlive/texmf-dist/tex/latex/listings/listings.sty
(/usr/share/texlive/texmf-dist/tex/latex/listings/lstmisc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/listings/listings.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/listings/lstlang1.sty)
(/usr/share/texlive/texmf-dist/tex/latex/preprint/balance.sty)
Excluding comment 'screenonly' Include comment 'printonly'
Include comment 'anonsuppress'/usr/bin/pygmentize
 (./main.aux)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/omlnxlmi.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/untxexa.fd)
(/usr/share/texlive/texmf-dist/tex/latex/base/ts1cmr.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/lmsntxsy.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/lmxntxexx.fd)
(/usr/share/texlive/texmf-dist/tex/latex/libertine/OT1LinuxLibertineT-TLF.fd)<<
ot1.cmap>><<oml.cmap>>
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/untxmia.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/untxsym.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/untxsyc.fd)
ABD: EveryShipout initializing macros
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))
(./main.out) (./main.out)
(/usr/share/texlive/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texlive/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(/usr/share/texlive/texmf-dist/tex/latex/libertine/T1LinuxBiolinumT-TLF.fd)
(/usr/share/texlive/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/microtype/mt-msb.cfg) (./abstract.tex
Excluding 'comment' comment.)

Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `\\' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `\\' on input line 158.

(./introduction.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 2.


Underfull \vbox (badness 5036) has occurred while \output is active [1.1{/var/l
ib/texmf/fonts/map/pdftex/updmap/pdftex.map}]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 47.


Underfull \vbox (badness 10000) has occurred while \output is active)
(./background.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 15.

(/usr/share/texlive/texmf-dist/tex/latex/inconsolata/t1zi4.fd)

pdfTeX warning: pdflatex (file ./csr.pdf): PDF inclusion: found PDF version <1.
7>, but at most version <1.5> allowed

Class acmart Warning: A possible image without description on input line 30.


LaTeX Warning: `!h' float specifier changed to `!ht'.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 35.

[2.2]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 42.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 42.

(./main.out.pyg) (./main.out.pyg) (./main.out.pyg)

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 48.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 74.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 74.

(./main.out.pyg)

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 84.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 86.



pdfTeX warning: pdflatex (file ./index_matching.pdf): PDF inclusion: found PDF 
version <1.7>, but at most version <1.5> allowed

Overfull \hbox (26.59892pt too wide) in paragraph at lines 93--96
 []|  [] 

Class acmart Warning: A possible image without description on input line 99.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 103.


Class acmart Warning: A possible image without description on input line 116.

[3.3 <./csr.pdf> <./index_matching.pdf

pdfTeX warning: pdflatex (file ./index_matching.pdf): PDF inclusion: multiple p
dfs with page group included in a single page
>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 121.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 123.

) (./overview.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 7.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 10.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 19.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 21.



pdfTeX warning: pdflatex (file ./overview_bitmap.pdf): PDF inclusion: found PDF
 version <1.7>, but at most version <1.5> allowed

Overfull \hbox (31.99515pt too wide) in paragraph at lines 29--32
 []|  [] 

Class acmart Warning: A possible image without description on input line 35.


LaTeX Warning: `!h' float specifier changed to `!ht'.


Underfull \vbox (badness 4001) has occurred while \output is active [4.4 <./opt
imal_indexing.pdf>]) (./mechanism.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 9.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 12.



pdfTeX warning: pdflatex (file ./bitmap_final.pdf): PDF inclusion: found PDF ve
rsion <1.7>, but at most version <1.5> allowed

Class acmart Warning: A possible image without description on input line 37.

[5.5 <./overview_bitmap.pdf> <./bitmap_final.pdf

pdfTeX warning: pdflatex (file ./bitmap_final.pdf): PDF inclusion: multiple pdf
s with page group included in a single page
>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 113.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `\newline' on input line 114.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 120.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 126.



pdfTeX warning: pdflatex (file ./bmu_overview.pdf): PDF inclusion: found PDF ve
rsion <1.7>, but at most version <1.5> allowed

Overfull \hbox (17.5091pt too wide) in paragraph at lines 134--137
 []|  [] 

Class acmart Warning: A possible image without description on input line 140.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 141.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 152.

[6.6 <./bmu_overview.pdf>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 187.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 253.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 255.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 287.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 290.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 292.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 294.



pdfTeX warning: pdflatex (file ./flow_spmv.pdf): PDF inclusion: found PDF versi
on <1.7>, but at most version <1.5> allowed

Class acmart Warning: A possible image without description on input line 313.


LaTeX Warning: `!h' float specifier changed to `!ht'.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 318.


Overfull \hbox (3.25229pt too wide) in paragraph at lines 334--335
[][][][][][][][][][][][][][][][][][][][][][]  

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 337.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 339.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 339.


LaTeX Warning: `!h' float specifier changed to `!ht'.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 357.

[7.7]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 433.


Underfull \vbox (badness 3514) has occurred while \output is active

pdfTeX warning: pdflatex (file ./flow_spmm.pdf): PDF inclusion: found PDF versi
on <1.7>, but at most version <1.5> allowed

Class acmart Warning: A possible image without description on input line 453.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 458.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 476.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 478.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 478.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 480.

) (./evaluation.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 4.


LaTeX Warning: `h' float specifier changed to `ht'.


LaTeX Warning: `h' float specifier changed to `ht'.


LaTeX Warning: `h' float specifier changed to `ht'.

[8.8 <./flow_spmv.pdf> <./flow_spmm.pdf

pdfTeX warning: pdflatex (file ./flow_spmm.pdf): PDF inclusion: multiple pdfs w
ith page group included in a single page
>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 141.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 162.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 165.


Class acmart Warning: A possible image without description on input line 191.


LaTeX Warning: `h' float specifier changed to `ht'.

[9.9]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 224.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 227.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 234.


Class acmart Warning: A possible image without description on input line 244.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 245.


Class acmart Warning: A possible image without description on input line 255.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 275.


Class acmart Warning: A possible image without description on input line 285.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 287.


Class acmart Warning: A possible image without description on input line 297.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 341.

[10.10 <./software.pdf> <./speedup_SpMV.pdf> <./instructions_SpMV.pdf> <./speed
up_SpMM.pdf> <./instructions_SpMM.pdf>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 371.


Class acmart Warning: A possible image without description on input line 382.


Class acmart Warning: A possible image without description on input line 391.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 406.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 423.


Class acmart Warning: A possible image without description on input line 432.


Class acmart Warning: A possible image without description on input line 441.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 518.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 521.


Class acmart Warning: A possible image without description on input line 537.

[11.11 <./granularity_spmv.pdf> <./granularity_spmm.pdf> <./locality_spmv.pdf> 
<./locality_spmm.pdf>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 555.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 557.


Class acmart Warning: A possible image without description on input line 573.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 611.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 614.


Class acmart Warning: A possible image without description on input line 632.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 653.

[12.12 <./graph.pdf> <./storage.pdf> <./conversion.pdf>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 656.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 666.

Excluding 'comment' comment.) (./related_work.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.

) (./conclusion.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.

[13.13]) (./acknowledgements.tex) (./main.bbl [14.14])

Class acmart Warning: Some images may lack descriptions.


Package balance Warning: You have called \balance in second column
(balance)                Columns might not be balanced.

[15.15] (./main.aux) )
(see the transcript file for additional information)pdfTeX warning (dest): name
{Hfootnote.1} has been referenced but does not exist, replaced by a fixed one

pdfTeX warning (dest): name{lstnumber.-2.17} has been referenced but does not e
xist, replaced by a fixed one

{/usr/share/texlive/texmf-dist/fonts/enc/dvips/newtx/libertinealt.enc}{/usr/sha
re/texlive/texmf-dist/fonts/enc/dvips/libertine/lbtn_25tcsq.enc}{/usr/share/tex
live/texmf-dist/fonts/enc/dvips/inconsolata/i4-t1-4.enc}{/usr/share/texlive/tex
mf-dist/fonts/enc/dvips/base/8r.enc}{/usr/share/texlive/texmf-dist/fonts/enc/dv
ips/libertine/lbtn_7grukw.enc}{/usr/share/texlive/texmf-dist/fonts/enc/dvips/li
bertine/lbtn_nh77jq.enc}{/usr/share/texlive/texmf-dist/fonts/enc/dvips/libertin
e/lbtn_oexx6f.enc}{/usr/share/texlive/texmf-dist/fonts/enc/dvips/libertine/lbtn
_76gpa5.enc}</usr/share/texlive/texmf-dist/fonts/type1/public/inconsolata/Incon
solata-zi4b.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/inconsolata/I
nconsolata-zi4r.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine
/LinBiolinumTB.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine/
LinBiolinumTI.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine/L
inLibertineT.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine/Li
nLibertineTB.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine/Li
nLibertineTI.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/newtx/fxlri-
7letters.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/txfonts/rtxmi.pf
b></usr/share/texlive/texmf-dist/fonts/type1/public/txfonts/rtxr.pfb></usr/shar
e/texlive/texmf-dist/fonts/type1/public/newtx/txexs.pfb></usr/share/texlive/tex
mf-dist/fonts/type1/public/newtx/txsys.pfb></usr/share/texlive/texmf-dist/fonts
/type1/public/newtx/zxlri.pfb>
Output written on main.pdf (15 pages, 1267602 bytes).
Transcript written on main.log.
pdflatex --shell-escape main.tex
This is pdfTeX, Version 3.14159265-2.6-1.40.19 (TeX Live 2019/dev/Debian) (preloaded format=pdflatex)
 \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2018-12-01>
(./acmart.cls
Document Class: acmart 2019/04/22 v1.60 Typesetting articles for the Associatio
n for Computing Machinery
(/usr/share/texlive/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/xkvutils.tex
(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/keyval.tex))))
(/usr/share/texlive/texmf-dist/tex/generic/xstring/xstring.sty
(/usr/share/texlive/texmf-dist/tex/generic/xstring/xstring.tex))
(/usr/share/texlive/texmf-dist/tex/latex/amscls/amsart.cls
Document Class: amsart 2017/10/31 v2.20.4
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/share/texlive/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/refcount.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ltxcmds.sty)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/infwarerr.sty))
(/usr/share/texlive/texmf-dist/tex/latex/totpages/totpages.sty
(/usr/share/texlive/texmf-dist/tex/latex/ms/everyshi.sty))
(/usr/share/texlive/texmf-dist/tex/latex/environ/environ.sty
(/usr/share/texlive/texmf-dist/tex/latex/trimspaces/trimspaces.sty))
(/usr/share/texlive/texmf-dist/tex/latex/textcase/textcase.sty)
(/usr/share/texlive/texmf-dist/tex/latex/natbib/natbib.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/share/texlive/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/share/texlive/texmf-dist/tex/latex/url/url.sty))
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texlive/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/share/texlive/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/geometry/geometry.sty)
(/usr/share/texlive/texmf-dist/tex/latex/ncctools/manyfoot.sty
(/usr/share/texlive/texmf-dist/tex/latex/ncctools/nccfoots.sty))
(/usr/share/texlive/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/share/texlive/texmf-dist/tex/generic/pdftex/glyphtounicode.tex)
(/usr/share/texlive/texmf-dist/tex/latex/cmap/cmap.sty)
(/usr/share/texlive/texmf-dist/tex/latex/base/fontenc.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/t1enc.def)<<t1.cmap>>)
(/usr/share/texlive/texmf-dist/tex/latex/libertine/libertine.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/textcomp.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/ts1enc.def
(/usr/share/texlive/texmf-dist/tex/latex/base/ts1enc.dfu)))
(/usr/share/texlive/texmf-dist/tex/latex/mweights/mweights.sty)
(/usr/share/texlive/texmf-dist/tex/latex/base/fontenc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/fontaxes/fontaxes.sty)
(/usr/share/texlive/texmf-dist/tex/latex/libertine/LinLibertine_I.tex))
(/usr/share/texlive/texmf-dist/tex/latex/inconsolata/zi4.sty
`inconsolata-zi4' v1.112, 2017/01/04 Text macros for Inconsolata (msharpe))
(/usr/share/texlive/texmf-dist/tex/latex/newtx/newtxmath.sty
`newtxmath' v1.553, 2018/05/15 Math macros based originally on txfonts (msharpe
) (/usr/share/texlive/texmf-dist/tex/latex/oberdiek/centernot.sty)
(/usr/share/texlive/texmf-dist/tex/generic/kastrup/binhex.tex))
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption.sty
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption3.sty))
(/usr/share/texlive/texmf-dist/tex/latex/float/float.sty)
(/usr/share/texlive/texmf-dist/tex/latex/comment/comment.sty
Excluding comment 'comment') Excluding comment 'CCSXML'
(/usr/share/texlive/texmf-dist/tex/latex/fancyhdr/fancyhdr.sty)
Special comment 'acks'
(/usr/share/texlive/texmf-dist/tex/latex/libertine/T1LinuxLibertineT-TLF.fd))
(/usr/share/texlive/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/share/texlive/texmf-dist/tex/latex/tools/calc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/share/texlive/texmf-dist/tex/latex/setspace/setspace.sty)
(/usr/share/texlive/texmf-dist/tex/latex/algorithms/algorithm.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/ifthen.sty))
(/usr/share/texlive/texmf-dist/tex/latex/algorithms/algorithmic.sty)
(/usr/share/texlive/texmf-dist/tex/latex/caption/subcaption.sty)
(/usr/share/texlive/texmf-dist/tex/latex/tools/array.sty)
(/usr/share/texlive/texmf-dist/tex/generic/ulem/ulem.sty)
(/usr/share/texlive/texmf-dist/tex/latex/minted/minted.sty
(/usr/share/texlive/texmf-dist/tex/latex/fvextra/fvextra.sty
(/usr/share/texlive/texmf-dist/tex/latex/fancyvrb/fancyvrb.sty
Style option: `fancyvrb' v3.2a <2019/01/15> (tvz))
(/usr/share/texlive/texmf-dist/tex/latex/upquote/upquote.sty)
(/usr/share/texlive/texmf-dist/tex/latex/lineno/lineno.sty))
(/usr/share/texlive/texmf-dist/tex/latex/tools/shellesc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/ifplatform/ifplatform.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/catchfile.sty) (./main.w18)
) (/usr/share/texlive/texmf-dist/tex/latex/framed/framed.sty)
(/usr/share/texlive/texmf-dist/tex/latex/caption/newfloat.sty))
(/usr/share/texlive/texmf-dist/tex/latex/tools/hhline.sty)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/frontendlayer/tikz.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-common-lists.t
ex)) (/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def
) (/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/pgf.revision.tex)))
(/usr/share/texlive/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeysfiltered.code.t
ex)) (/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.def
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-pdf.de
f)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.code.
tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigonomet
ric.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.random.cod
e.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.comparison
.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integerari
thmetics.code.tex)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconstruct.
code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicstate.c
ode.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransformation
s.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.code.tex
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.code.t
ex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathprocessing
.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.code.tex
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.code.tex

(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.code.
tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.code.te
x)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransparency.c
ode.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorerdf.code.tex))
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.code.tex
) (/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.tex
)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-0-65
.sty)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-1-18
.sty)) (/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgffor.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgfkeys.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex))
(/usr/share/texlive/texmf-dist/tex/latex/pgf/math/pgfmath.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgffor.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/tikz.code.tex

(/usr/share/texlive/texmf-dist/tex/generic/pgf/libraries/pgflibraryplothandlers
.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmodulematrix.code.tex
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tik
zlibrarytopaths.code.tex)))
(/usr/share/texlive/texmf-dist/tex/latex/mdframed/mdframed.sty
(/usr/share/texlive/texmf-dist/tex/latex/l3packages/xparse/xparse.sty
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/expl3.sty
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/expl3-code.tex)
(/usr/share/texlive/texmf-dist/tex/latex/l3kernel/l3pdfmode.def)))
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/zref-abspage.sty
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/zref-base.sty))
(/usr/share/texlive/texmf-dist/tex/latex/needspace/needspace.sty)
(/usr/share/texlive/texmf-dist/tex/latex/mdframed/md-frame-0.mdf))
(/usr/share/texlive/texmf-dist/tex/latex/makecell/makecell.sty)
(/usr/share/texlive/texmf-dist/tex/latex/dblfloatfix/dblfloatfix.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

)) (/usr/share/texlive/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/share/texlive/texmf-dist/tex/latex/tools/afterpage.sty)
(/usr/share/texlive/texmf-dist/tex/latex/listings/listings.sty
(/usr/share/texlive/texmf-dist/tex/latex/listings/lstmisc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/listings/listings.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/listings/lstlang1.sty)
(/usr/share/texlive/texmf-dist/tex/latex/preprint/balance.sty)
Excluding comment 'screenonly' Include comment 'printonly'
Include comment 'anonsuppress'/usr/bin/pygmentize
 (./main.aux)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/omlnxlmi.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/untxexa.fd)
(/usr/share/texlive/texmf-dist/tex/latex/base/ts1cmr.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/lmsntxsy.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/lmxntxexx.fd)
(/usr/share/texlive/texmf-dist/tex/latex/libertine/OT1LinuxLibertineT-TLF.fd)<<
ot1.cmap>><<oml.cmap>>
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/untxmia.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/untxsym.fd)
(/usr/share/texlive/texmf-dist/tex/latex/newtx/untxsyc.fd)
ABD: EveryShipout initializing macros
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))
(./main.out) (./main.out)
(/usr/share/texlive/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texlive/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(/usr/share/texlive/texmf-dist/tex/latex/libertine/T1LinuxBiolinumT-TLF.fd)
(/usr/share/texlive/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/microtype/mt-msb.cfg) (./abstract.tex
Excluding 'comment' comment.)

Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `superscript' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `math shift' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `\\' on input line 158.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `\\' on input line 158.

(./introduction.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 2.


Underfull \vbox (badness 5036) has occurred while \output is active [1.1{/var/l
ib/texmf/fonts/map/pdftex/updmap/pdftex.map}]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 47.


Underfull \vbox (badness 10000) has occurred while \output is active)
(./background.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 15.

(/usr/share/texlive/texmf-dist/tex/latex/inconsolata/t1zi4.fd)

pdfTeX warning: pdflatex (file ./csr.pdf): PDF inclusion: found PDF version <1.
7>, but at most version <1.5> allowed

Class acmart Warning: A possible image without description on input line 30.


LaTeX Warning: `!h' float specifier changed to `!ht'.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 35.

[2.2]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 42.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 42.

(./main.out.pyg) (./main.out.pyg) (./main.out.pyg)

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 48.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 74.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 74.

(./main.out.pyg)

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 84.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 86.



pdfTeX warning: pdflatex (file ./index_matching.pdf): PDF inclusion: found PDF 
version <1.7>, but at most version <1.5> allowed

Overfull \hbox (26.59892pt too wide) in paragraph at lines 93--96
 []|  [] 

Class acmart Warning: A possible image without description on input line 99.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 103.


Class acmart Warning: A possible image without description on input line 116.

[3.3 <./csr.pdf> <./index_matching.pdf

pdfTeX warning: pdflatex (file ./index_matching.pdf): PDF inclusion: multiple p
dfs with page group included in a single page
>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 121.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 123.

) (./overview.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 7.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 10.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 19.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 21.



pdfTeX warning: pdflatex (file ./overview_bitmap.pdf): PDF inclusion: found PDF
 version <1.7>, but at most version <1.5> allowed

Overfull \hbox (31.99515pt too wide) in paragraph at lines 29--32
 []|  [] 

Class acmart Warning: A possible image without description on input line 35.


LaTeX Warning: `!h' float specifier changed to `!ht'.


Underfull \vbox (badness 4001) has occurred while \output is active [4.4 <./opt
imal_indexing.pdf>]) (./mechanism.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 9.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 12.



pdfTeX warning: pdflatex (file ./bitmap_final.pdf): PDF inclusion: found PDF ve
rsion <1.7>, but at most version <1.5> allowed

Class acmart Warning: A possible image without description on input line 37.

[5.5 <./overview_bitmap.pdf> <./bitmap_final.pdf

pdfTeX warning: pdflatex (file ./bitmap_final.pdf): PDF inclusion: multiple pdf
s with page group included in a single page
>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 113.


Package hyperref Warning: Token not allowed in a PDF string (Unicode):
(hyperref)                removing `\newline' on input line 114.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 120.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 126.



pdfTeX warning: pdflatex (file ./bmu_overview.pdf): PDF inclusion: found PDF ve
rsion <1.7>, but at most version <1.5> allowed

Overfull \hbox (17.5091pt too wide) in paragraph at lines 134--137
 []|  [] 

Class acmart Warning: A possible image without description on input line 140.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 141.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 152.

[6.6 <./bmu_overview.pdf>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 187.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 253.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 255.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 287.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 290.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 292.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 294.



pdfTeX warning: pdflatex (file ./flow_spmv.pdf): PDF inclusion: found PDF versi
on <1.7>, but at most version <1.5> allowed

Class acmart Warning: A possible image without description on input line 313.


LaTeX Warning: `!h' float specifier changed to `!ht'.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 318.


Overfull \hbox (3.25229pt too wide) in paragraph at lines 334--335
[][][][][][][][][][][][][][][][][][][][][][]  

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 337.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 339.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 339.


LaTeX Warning: `!h' float specifier changed to `!ht'.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 357.

[7.7]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 433.


Underfull \vbox (badness 3514) has occurred while \output is active

pdfTeX warning: pdflatex (file ./flow_spmm.pdf): PDF inclusion: found PDF versi
on <1.7>, but at most version <1.5> allowed

Class acmart Warning: A possible image without description on input line 453.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 458.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 476.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 478.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 478.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 480.

) (./evaluation.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 4.


LaTeX Warning: `h' float specifier changed to `ht'.


LaTeX Warning: `h' float specifier changed to `ht'.


LaTeX Warning: `h' float specifier changed to `ht'.

[8.8 <./flow_spmv.pdf> <./flow_spmm.pdf

pdfTeX warning: pdflatex (file ./flow_spmm.pdf): PDF inclusion: multiple pdfs w
ith page group included in a single page
>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 141.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 162.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 165.


Class acmart Warning: A possible image without description on input line 191.


LaTeX Warning: `h' float specifier changed to `ht'.

[9.9]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 224.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 227.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 234.


Class acmart Warning: A possible image without description on input line 244.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 245.


Class acmart Warning: A possible image without description on input line 255.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 275.


Class acmart Warning: A possible image without description on input line 285.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 287.


Class acmart Warning: A possible image without description on input line 297.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 341.

[10.10 <./software.pdf> <./speedup_SpMV.pdf> <./instructions_SpMV.pdf> <./speed
up_SpMM.pdf> <./instructions_SpMM.pdf>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 371.


Class acmart Warning: A possible image without description on input line 382.


Class acmart Warning: A possible image without description on input line 391.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 406.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 423.


Class acmart Warning: A possible image without description on input line 432.


Class acmart Warning: A possible image without description on input line 441.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 518.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 521.


Class acmart Warning: A possible image without description on input line 537.

[11.11 <./granularity_spmv.pdf> <./granularity_spmm.pdf> <./locality_spmv.pdf> 
<./locality_spmm.pdf>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 555.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 557.


Class acmart Warning: A possible image without description on input line 573.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 611.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 614.


Class acmart Warning: A possible image without description on input line 632.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 653.

[12.12 <./graph.pdf> <./storage.pdf> <./conversion.pdf>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 656.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 666.

Excluding 'comment' comment.) (./related_work.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.

) (./conclusion.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 1.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.

[13.13]) (./acknowledgements.tex) (./main.bbl [14.14])

Class acmart Warning: Some images may lack descriptions.


Package balance Warning: You have called \balance in second column
(balance)                Columns might not be balanced.

[15.15] (./main.aux) )
(see the transcript file for additional information)pdfTeX warning (dest): name
{Hfootnote.1} has been referenced but does not exist, replaced by a fixed one

pdfTeX warning (dest): name{lstnumber.-2.17} has been referenced but does not e
xist, replaced by a fixed one

{/usr/share/texlive/texmf-dist/fonts/enc/dvips/newtx/libertinealt.enc}{/usr/sha
re/texlive/texmf-dist/fonts/enc/dvips/libertine/lbtn_25tcsq.enc}{/usr/share/tex
live/texmf-dist/fonts/enc/dvips/inconsolata/i4-t1-4.enc}{/usr/share/texlive/tex
mf-dist/fonts/enc/dvips/base/8r.enc}{/usr/share/texlive/texmf-dist/fonts/enc/dv
ips/libertine/lbtn_7grukw.enc}{/usr/share/texlive/texmf-dist/fonts/enc/dvips/li
bertine/lbtn_nh77jq.enc}{/usr/share/texlive/texmf-dist/fonts/enc/dvips/libertin
e/lbtn_oexx6f.enc}{/usr/share/texlive/texmf-dist/fonts/enc/dvips/libertine/lbtn
_76gpa5.enc}</usr/share/texlive/texmf-dist/fonts/type1/public/inconsolata/Incon
solata-zi4b.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/inconsolata/I
nconsolata-zi4r.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine
/LinBiolinumTB.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine/
LinBiolinumTI.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine/L
inLibertineT.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine/Li
nLibertineTB.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/libertine/Li
nLibertineTI.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/newtx/fxlri-
7letters.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/txfonts/rtxmi.pf
b></usr/share/texlive/texmf-dist/fonts/type1/public/txfonts/rtxr.pfb></usr/shar
e/texlive/texmf-dist/fonts/type1/public/newtx/txexs.pfb></usr/share/texlive/tex
mf-dist/fonts/type1/public/newtx/txsys.pfb></usr/share/texlive/texmf-dist/fonts
/type1/public/newtx/zxlri.pfb>
Output written on main.pdf (15 pages, 1267602 bytes).
Transcript written on main.log.

